Deep Curvature Suite

We present MLRG Deep Curvature suite, a PyTorch-based, open-source package for analysis and visualisation of neural network curvature and loss landscape. Despite of providing rich information into properties of neural network and useful for a various designed tasks, curvature information is still not made sufficient use for various reasons, and our method aims to bridge this gap. We present a primer, including its main practical desiderata and common misconceptions, of \textit{Lanczos algorithm}, the theoretical backbone of our package, and present a series of examples based on synthetic toy examples and realistic modern neural networks tested on CIFAR datasets, and show the superiority of our package against existing competing approaches for the similar purposes.

==> experiments.tex <==
\section{Experiments}
%Through the use of experiments on a simple 9 layers convolutional neural networks  and ResNet-18, we test our two main theoretical contributions: 

We organized our experiments as follows. We first validate the theory derived from Section\ref{sec:spectralimplication} in \ref{ssec:val}. Then from the equation we derived in Section\ref{sec:quadraticformulae} we experiment a new optimizer based on the optimal values of Eq.\ref{eq:alphaandbeta}.

\subsection{Validation of the theory}\label{ssec:val}
In this subsection, two of our main contributions:
\begin{itemize}
    \item Whether the number of outlier eigenvalues in the Gauss-Newton spectrum is well approximated by the number of layers;
    \item Whether the mean of the bulk is a better approximation to the underlying convex surrogate objective, as opposed to the sample-estimated smallest eigenvalue.
\end{itemize}

\paragraph{Learning the loss with Lanczos}
In order to investigate the stability of the Hessian for large neural networks and avoid the costly $\mathcal{O}(n^{3})$ eigen-decompostion and $\mathcal{O}(n^{2})$ storage we implement the Lanczos algorithm \cite{meurant2006lanczos}  with the Pearlmutter trick \cite{pearlmutter1994fast} with computational and storage cost $\mathcal{O}(mn)$, where $m$ is the number of Lanczos steps taken. Beyond having improved convergence to the power iteration method \footnote{For an eigengap $\rho = \lambda_{1}/\lambda_{2}$ the power iteration converges to the top eigenvalue/eigenvector pair as $1+2\rho$ and Lanczos as $1 + 2\rho + 2\sqrt{\rho^{2}+\rho}$} \cite{bai1996some} it further produces estimates of eigenvectors and eigenvalues other than that corresponding to the largest eigenvalue, known as Ritz values/vectors. The Lanczos tri-diagonal matrix $\mathbb{T}$ can be derived from the Moment matrix $M_{ij} = v^{T}H^{i+j-2}v$ where $H$ is the absolute Hessian or GGN in our case, corresponding to the discrete measure $d\alpha(\lambda)$ satisfying the moments $\mu_{i} = v^{T}H^{i}v = \int \lambda^{i}d\alpha(\lambda)$ \cite{golub1994matrices}. For zero mean unit variance random vectors $v$,%\footnote{NB: This does not hold for any vector it must be zero mean}
the non-central moments of the Hessian spectral density can be written as \cite{ete},
\begin{equation}
\mathbb{E}_{v}(v^{T} H^{m} v) = \sum_{i=1}^{n}\lambda_{i}^{m} \approx \frac{1}{n_{v}}\sum_{j=1}^{n_{v}}v_{j}^{T}Hv_{j},
\end{equation}
Hence, the eigenvector/eigenvalue pairs of $\mathbb{T}$ contain information about the spectral density of $H$ %\footnote{Unless the vectors are re-orthogonalised the quality of this spectral approximation quickly degrades}. 
For $n_{v}$ starting vectors, the corresponding discrete spectral density is given as,
\begin{equation}
\label{eq:spectraldensitymanyseeds}
p(\lambda) = \frac{1}{n_{v}}\sum_{l=1}^{n_{v}}\biggl(\sum_{k=1}^{m}(\tau_{k}^{(l)})^{2}\delta(\lambda-\lambda_{k}^{(l)})\biggr),
\end{equation}
where $\tau_{k}^{(l)}$ corresponds to the first entry of the eigenvector of the $k$-th eigenvalue, $\lambda_{k}$, of the Lanczos tri-diagonal matrix, $\mathbb{T}$, for the $l$-th starting vector \cite{ubaruapplications, lin2016approximating}.

For the experiments in Sec~\ref{ssec:application}, we reduced the storage cost of our procedure from $\mathcal{O}(mn) \rightarrow \mathcal{O}(n)$ by removing Lanczos orthogonalisation and re-using the gradient vector instead of a random vector. The gradient is not guaranteed to be zero mean and hence we cannot learn the spectral density of the surrogate Hessian directly. However, given the arguments in Sec~\ref{sec:theoreticalcontribution}, if we discount the Ritz value of smallest absolute magnitude pertaining to the excess zero mode and remove the top $j$ eigenvalues given by the number of layers, the median of the remaining Ritz eigenvalues \footnote{as long as $m>>j$} will be an effective approximation of the mean of the bulk. We show this on a synthetic example where we generated the eigenspectrum of a matrix $G = VDV^{-1} \in \mathcal{R}^{3000\times 3000}$ where $D$ is the diagonal eigenvalue matrix and $V$ is a matrix orthonormal random vectors. We generate a synthetic eigenspectrum with $2500$ zeros, $480$ drawn uniformly over $[0,10]$ and $20$ uniformly over $[0,300]$. We compare the procedure described in this paragraph which we named Ritz in Table~\ref{table:learnusingmedian}(which removed the excess zero mode and the outliers) and compared to just using the median of the Ritz values to the known ground truth of $5$. We run the experiment $300$ times and quote the results in Table \ref{table:learnusingmedian}. Here we see that the median seems to be an effective approximation to the result from a random vector and summarise the steps for use in Algorithm \ref{alg:learnmeanbulkapprox}.

\begin{algorithm}[tb]
	\caption{Mean of the Bulk with Gradient vector}
	\label{alg:learnmeanbulkapprox}
	\begin{algorithmic}
		\STATE {\bfseries Input:} Lanczos Ritz-values/vectors $\lambda_{i} \forall i \leq m$, number of Layers $l$
		\STATE {\bfseries Output:} $\lambda_{b} = \lambda_{m-l-1/2}$
		%\STATE {\bfseries Output:} $\lambda_{b} = \frac{\sum_{i}_{3}^{m-l}\lambda_{i}}{m-l-2}$
	\end{algorithmic}
\end{algorithm}

\begin{table}[htb!]
\caption{Estimation of the bulk mean using different algorithms, the target Mean value is 5.} \label{table:learnusingmedian}
\begin{center} 
\begin{tabular}{ccccccc}
\toprule
         & Random Vector & Ritz  & Median \\ \midrule
Mean     &           5.0119        & 5.33   & 5.1719 \\ \midrule
Variance &           0.258         & 0.1817 & 0.0436 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

\paragraph{Gauss-Newton outliers: Eigenspectrum for networks on CIFAR-10} \label{subsec:eigspec_on_cifar10}
In this section we studied the evolution of the Hessian spectrum of a basic deep neural network during traininghessian. The network referred as BasicNet in this paper consists of 8 convolutions followed by ReLU activations, $3\times 3$ max-pooling layers with stride 2 after each of the first $3$ activations. We tried variants of this network with and without batch-normalisation \cite{ioffe2015batch}
We use $n_{v} = 5$ random Gaussian seed vectors with $m=200$ Lanczos steps, a batch size of $T = 128$ and train on the CIFAR-10 classification dataset. The total number of layers, summing convolutional, max-pooling and output are $m = 8$. We run SGD with a learning rate $\alpha = 0.001$ and Momentum $\beta = 0.9$. We plot the results of equation \ref{eq:spectraldensitymanyseeds} with and without Batch Normalization as a stem graph in Figure \ref{fig:cifarBN_1_vary_x}. We note that key spectral characteristics remain unchanged across several epochs. Primarily the majority of the spectral mass $>99\%$ is located at the Ritz value closest to $0$, given the low rank nature of the empirical Gauss-Newton. This is unsurprising and hence this peak is omitted in the plots for clarity. Furthermore, the remaining spectral mass is largely comprised of a spectral bulk which spreads out from the origin and is well modelled by the Marcenko-Pastur distribution (fitted in red), then there are a few large outliers well-separated from the bulk. This corroborates results noted in smaller networks by earlier work \cite{sagun2016eigenvalues,sagun2017empirical} and grounds the validity of our assumptions\cite{S:which assumption? If it's the RMT theory where did you state it clearly?}.

%%------ Figure 2 varying x scale initial training ----------%%
\begin{figure}[htb!]
	\centering
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.3cm 0cm 0.1cm 0.0cm, clip, width=1.0\linewidth]{figures/vary_x_scale/cifarnobn_GN_mean_EigSpec_Itr0.png}
		\caption{No BN: Iteration 0}
	\end{subfigure}
	\hspace{5pt}
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.3cm 0cm 0.1cm 0.0cm, clip, width=1.0\linewidth]{figures/vary_x_scale/cifarbn_GN_mean_EigSpec_Itr0.png}
		\caption{BN: Iteration 0}	
	\end{subfigure}%
	\vspace{5pt}
	
	\begin{subfigure}{0.45\linewidth}
		\centering
		% 		 trim={<left> <lower> <right> <upper>}
		\includegraphics[trim=0.3cm 0cm 0.1cm 0.0cm, clip, width=1.0\linewidth]{figures/vary_x_scale/cifarnobn_GN_mean_EigSpec_Itr1872.png}
		\caption{No BN: Iteration 1872}	
	\end{subfigure}%
	\hspace{5pt}
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.3cm 0cm 0.1cm 0.0cm, clip, width=1.0\linewidth]{figures/vary_x_scale/cifarbn_GN_mean_EigSpec_Itr1872.png}
		\caption{BN: Iteration 1872}	
	\end{subfigure}%
	\vspace{5pt}
	
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.3cm 0cm 0.1cm 0.0cm, clip, width=1.0\linewidth]{figures/vary_x_scale/cifarnobn_GN_mean_EigSpec_Itr3744.png}
		\caption{No BN: Iteration 3744}	
	\end{subfigure}%
	\hspace{5pt}
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.3cm 0cm 0.1cm 0.0cm, clip, width=1.0\linewidth]{figures/vary_x_scale/cifarbn_GN_mean_EigSpec_Itr3744.png}
		\caption{BN: Iteration 3744}
	\end{subfigure}%
	\vspace{5pt}
	\caption{Eigen-spectra of Gauss-Newton Matrices for BasicNet over Cifar-10, trained using SGD with learning rate of $0.001$. The left column shows the results \textbf{without batch norm (No BN)}. The right column shows the results \textbf{with batch norm (BN)}. The above plots shows the change of the spectra over the \textbf{first} $3744$ training iterations.}
	\label{fig:cifarBN_1_vary_x}
\end{figure}
The number of outliers in Figures \ref{fig:cifarBN_1_vary_x} remains remarkably consistent. Whilst more clearly visible without batch-normalization, it remains $\mathcal{O}(10)$ for both, consistent with the estimation of $m=8$ from Section \ref{ssec:outliernumber}. 
\begin{figure}
    \centering
		\includegraphics[trim=0cm 0.cm 0cm 0cm, clip, width=0.9\linewidth]{figures/resnet-spectrum__GN_EigSpec_Itr0_modi.eps}
		\caption{Eigenvalue spectrum of ResNet-18 at training iteration 0 which contains $18$ outliers and a bulk fitted with Marchenko-Pastur distribution.}
    \label{fig:ResNet18spectra}
\end{figure}
\begin{table}[htb!]
\caption{The number of outliers in the eigenvalue spectra of ResNet-18 over training iterations} \label{table:outlier_number_over_itr}
\begin{center} 
    \begin{tabular}{ccccccc}
    \toprule 
    Iteration steps & 0 & 22464 & 33696 & 41184 \\\midrule
    Number of Outliers & 18 & 16 & 20 & 21 \\ 
    \bottomrule
    \end{tabular}
\end{center}
\end{table}
We also test a ResNet-18 using batch-norm and find similarly to the BasicNet, that the number of outliers, shown by a gap in the Ritz values, is consistent with the number of layers $m=18$. Shown in Figure \ref{fig:ResNet18spectra}. We repeat the results for the ResNet-18 with the standard learning rate of $0.1$ and find identical results. For consistency We estimate the outlier number using Algorithm \ref{alg:outlierlearner1}, but note that as the Ritz values do not arrive top down and that along with the dependence on the tolerance $c$ this is an ineffective way to learn the number of outliers online, hence motivating Algorithm \ref{alg:learnmeanbulk}.
\begin{algorithm}[htb!]
	\caption{Outlier learner}
	\label{alg:outlierlearner1}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} Lanczos Ritz-values:  $\{ \lambda_i \}_{i=1}^k$  with $\lambda_1 > \dots > \lambda_k $ and a threshold value $c$
% 		\STATE Obtain $\hat{\lambda}_i$ by removing the mass at the $0$ from the $\lambda_i$
		\STATE Compute $\{ \Delta \lambda_i \}_{i=1}^{k-1}$ where $ \Delta \lambda_i = \frac{(\lambda_i - \lambda_{i-1})}{\lambda_1}$
		\STATE Find $i^*= \argmax_{i \in \{1, \dots, k-1 \}} \left[ \Delta \lambda_i \geq c \right] $
		\STATE {\bfseries Output:} Number of outliers $N_o =i^* $ 
	\end{algorithmic}
\end{algorithm}


\paragraph{Effect of the mean bulk hypothesis in optimization}
In order to test our hypothesis about the importance of correcting for the finite sample effects in Section \ref{sec:spectralimplication}. We run our optimization algorithims as before but instead of using the mean of the bulk, we instead use the second smallest Ritz value. We use the second because the first corresponds to the enormous excess zero mode, as described in section $\ref{subsec:ghosts}$. We plot the results for the BasicNet and ResNet, training and validation in Figures \ref{fig:basicnet_resnet_lowvshigh}. The dashed $-L$ denotes the use of Low momentum, which comes from us using the median of the bulk and the dashed, $-H$ denotes High momentum, because we use the second smallest Ritz value in Figure \ref{fig:basicnet_resnet_lowvshigh} and hence the value of momentum calculated from Equation \eqref{eq:alphaandbeta} is higher. As can be clearly seen the training and validation loss for all positive definite approximations and for all architectures is much improved when using the mean of the bulk, lending credence to the practical value of our theoretical arguments in Section \ref{sec:theoreticalcontribution}.
\begin{figure}[htb!]
	\centering
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.0cm 0cm 0.0cm 0.0cm, clip, width=1.0\linewidth]{figures/CIFAR10_BasicNet_BN_trainLH.eps}
		\caption{BasicNet training}
	\end{subfigure}
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.0cm 0cm 0.0cm 0.0cm, clip, width=1.0\linewidth]{figures/CIFAR10_BasicNet_BN_validLH.eps}
		\caption{BasicNet Validation}	
	\end{subfigure}%
	
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.0cm 0cm 0.0cm 0.0cm, clip, width=1.0\linewidth]{figures/CIFAR10_ResNet_BN_trainLH.eps}
		\caption{ResNet training}
	\end{subfigure}
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.0cm 0cm 0.0cm 0.cm, clip, width=1.0\linewidth]{figures/CIFAR10_ResNet_BN_validLH.eps}
		\caption{ResNet validation}	
	\end{subfigure}
	
	\caption{The effect of using low momentum and high momentum on training and validation loss of the BasicNet and the ResNet-18.}
	\label{fig:basicnet_resnet_lowvshigh}
\end{figure}


\section{On the Gradient Perturbation}
Let us consider the $j$'th component of the difference vector between the gradients of the true and empirical risks at a point in weight space $w$
\begin{equation}
\epsilon(w)_{j} = \nabla_{j} R_{true} - \nabla_{j} R_{emp} = \mathbb{E}[\nabla_{j} l(h(x;w),y)] - \frac{1}{T}\sum_{i=1}^{T}\nabla_{j} l(h(x_{i};w),y_{i})
\end{equation}
For any $P(x,y)$, such that the moments $\mathbb{E}[\nabla_{j} l(h(x;w),y)]^{m}$ are bounded and with sufficient independence between the samples \cite{stein1972}, in the limit $T\rightarrow \infty$ this converges almost surely to a normal random variable. Let us for simplicity assume that the samples are independent and unbiased, such that we converge to $\epsilon(w)_{j} \sim \mathcal{N}(0,\frac{\sigma_{j}^{2}}{T})$. Assuming independence between gradient components, The $L2$ norm squared of the vector $|\epsilon(w)|^{2} = \sum_{j=1}^{N} [\epsilon_{j}(w)]^{2}$ can be seen as the sum of $N$ normally distributed random variables which, again using the independence assumption between gradient components, gives a Chi-Square distribution, with corresponding mean $\frac{1}{T} \sum_{j=1}^{N}\sigma_{j}^{2}$ and hence an $L2$ norm of $\sqrt{\frac{N}{T} \langle\sigma_{j}^{2}\rangle}$ where we have used $\langle\sigma_{j}^{2}\rangle = \sum_{j=1}^{N}\sigma_{j}^{2}/N$. In general we do not expect $\sigma_{j} = 0$. For large $q = N/T$, This can lead to problems in areas of the loss landscape where $\nabla L_{true} = 0$ as $|\epsilon|$ may be non negligible, limiting our ability to hone in to the region of the weight space where the model will perform best on in expectation on samples from the data generating distribution, i.e unseen data. Relaxing the assumptions on sample independence, gives us a $T_{eff} < T$, which worsens this perturbation. Relaxing the assumption on gradient component independence simply affects our weightings of the various $\sigma_{j}^{2}$ components and does not affect the sum in $N$.

% \subsection{Estimating the Noise}
% writing the gradient of a batch as the true gradient at that point in weight space and a realization of a random variable
% \begin{equation}
%     \nabla L_{1} = \nabla L_{true} + \eta_{1}
% \end{equation}
% we have by extension
% \begin{equation}
% \label{eq:trueestimategradient}
%     \frac{\sum_{i\neq j}^{m}\nabla L_{i}^{T}\nabla L_{j}}{\sum_{i}^{m}\nabla L_{i}^{T}\nabla L_{i}} = \frac{\sum_{i\neq j}^{m}\nabla L_{true}^{T}\nabla L_{true} + \eta_{i}^{T}\eta_{j} + \nabla L_{true}^{T}(\eta_{i}+\eta_{j})}{\sum_{i}^{m}\nabla L_{true}^{T}\nabla L_{true} + \eta_{i}^{T}\eta_{i} + 2\nabla L_{true}^{T}\eta_{i}} 
% \end{equation}
% (CHECK THIS). As the elements of the vector $\eta_{i}$ are given by a gaussian random variable, the vector is a gaussian random vector (NOT SURE ABOUT THE DIFFERENT VARIANCES) and we have by extension the fact that in high dimensions (GET ACTUAL RESULTS FOR THIS), the root mean square overlap of two random vectors goes as $1/\sqrt{N}$. More importantly for the second term in the numerator of \eqref{eq:trueestimategradient} the product of two independent normal variables is still a normal variable, and the sum of a normal variables is also a normal variable and hence as they are all $0$ mean it is still zero mean. Similiarly for the third term in the numerator and in the denominator, the gaussian random vector is rotationally invariant and hence in expectation these terms are also zero. This leaves us with
% \begin{equation}
% \label{eq:gradientsimplified}
%     \frac{\sum_{i\neq j}^{m}\nabla L_{i}^{T}\nabla L_{j}}{\sum_{i}^{m}\nabla L_{i}^{T}\nabla L_{i}} = \frac{\sum_{i\neq j}^{m}\nabla L_{true}^{T}\nabla L_{true}}{\sum_{i}^{m}\nabla L_{true}^{T}\nabla L_{true} + \eta_{i}^{T}\eta_{i}} 
% \end{equation}
\subsection{Stochastic Weight Averaging and the true risk optimum}
For a convex true risk function with Lipshitz bound $\beta$.
Using the Lipschitz and convexity properties, and assuming a learning rate $\eta_{t} < 1/\beta$ as detailed in Appendix \ref{stochderivation}, we can rewrite the difference between the true risk at the $t+1$'th iterate and optimal value as
\begin{equation}
\begin{aligned}
l(w_{t+1})-l(w^{*}) % & \leq -\epsilon(w)_{t}(w_{t}-w^{*}) -\eta_{t}(-\epsilon(w)_{t})(\nabla l(w_{t})+\epsilon(w)_{t}) \\  & +\frac{1}{2\eta_{t}}(||w_{t}-w^{*}||^{2}-||x_{t+1}-w^{*}||^{2}) \\ 
& \leq -\epsilon(w)_{t}\bigg((w_{t}-w^{*})-\eta_{t} \nabla l(w_{t})\bigg) + \eta_{t} ||\epsilon(w)_{t}||^{2} \\ & +\frac{1}{2\eta_{t}}(||w_{t}-w^{*}||^{2}-||w_{t+1}-w^{*}||^{2}) \\ 
\end{aligned}
\end{equation}
%As discussed each component of $\epsilon(w)_{t}$ is the realization of a zero mean normal random variable with variance $\sigma_{i}^{2}$, hence the variance of the first bracketed term in each component goes as $|w_{t}-w^{*}|^{2}_{i}+\eta^{2}|\nabla l(w_{t})|^{2}_{i}$. Summing from $t=1$ to $t=n$. We have
%\begin{equation}
%\begin{aligned}
%& \frac{1}{n}\sum_{i=1}^{n}l(w_{t+1})-l(w^{*})  \leq f(\frac{1}{n}\sum_{i=1}^{n}x_{t+1}))-l(w^{*}) \\ 
%& \leq \frac{1}{n}\sum_{t=1}^{n}\bigg(-\epsilon(w)_{t}\bigg((w_{t}-w^{*})-\eta_{t} \nabla l(w_{t})\bigg) + \eta_{t} ||\epsilon(w)_{t}||^{2} +\frac{1}{2\eta_{t}}(||w_{t}-w^{*}||^{2}-||x_{t+1}-w^{*}||^{2}) \bigg) \\ 
%\end{aligned}
%\end{equation}
%Looking exclusively at the third term in the sum, we have
%\begin{equation}
%\frac{1}{2\eta_{1}}||x_{1}-w^{*}||^{2}+\sum_{i=2}^{n}(\frac{1}{2\eta_{t}}-\frac{1}{2\eta_{t-1}})||w_{t}-w^{*}||^{2}-\frac{1}{\eta_{t}}||x_{t+1}-w^{*}||^{2}
%\end{equation}
%Dropping the last term (as it is negative) and by noting that the $\eta_{t}>\eta_{t+1}$ we replace the square term in the sum by an upper bound $R^{2}$, and also in the first term, giving
Using the convexity of functions, summing the iterates and bounding the components of the telescopic sum
\begin{equation}
\label{eq:mainoptimisationbeast}
\begin{aligned}
& \frac{1}{n}\sum_{i=1}^{n}l(w_{t+1})-l(w^{*})  \leq l(\frac{1}{n}\sum_{i=1}^{n}x_{t+1}))-l(w^{*}) \\ 
& \leq \frac{1}{n}\sum_{t=1}^{n}\bigg[-\epsilon(w)_{t}\bigg((w_{t}-w^{*})-\eta_{t} \nabla l(w_{t})\bigg)\bigg] +\frac{1}{n}\sum_{t=1}^{n} \bigg(\eta_{t}||\epsilon(w)_{t}||^{2}+ \frac{R^{2}}{2\eta_{t}}\bigg) \\ 
\end{aligned}
\end{equation}
The second part is typically studied in stochastic gradient descent, where $\epsilon(t)$ is considered as a perturbation to the full dataset empirical gradient when only a sub-sample is taken, its expectation with respect to the dataset $\mathbb{E}(\epsilon(w)_{t}) = 0$ and hence in expectation the first term vanishes. This allows us to take an $\eta_{t} \propto t^{-1/2}$ establishing convergence for the iterate sum. We note that no such proof of convergence exists for the final iterate \cite{duchi2018introductory}. 
\begin{center}
	\centering
\begin{tikzpicture}
\label{vectoroverlap}
\draw[thin,gray!40] (-2,-2) grid (2,2);
%\draw[<->] (-2,0)--(2,0) node[right]{$x$};
%\draw[<->] (0,-2)--(0,2) node[above]{$y$};
\draw[line width=2pt,blue,-stealth](-2,-2)--(0,1) node[anchor=east]{$\boldsymbol{g_{emp}}$};
\draw[line width=2pt,red,-stealth](-2,-2)--(1,0) node[anchor=north west]{$\boldsymbol{g_{t}}$};
\draw[line width=2pt,black,-stealth](1,0)--(0,1) node[anchor=south west]{$\boldsymbol{\epsilon}$};
\end{tikzpicture}
\end{center}


for simplicity of notation, let us collect the term into the left hand side 
\begin{equation}
g(w_{t}) = w_{t}- \eta_{t}\nabla l(w_{t}) -w^{*}  = w^{opt}_{t+1}-w*
\end{equation}
The term on the left hand side an be written as 
\begin{equation}
|g(w_{t}) ||\epsilon(w_{t})|\cos \theta_{t}
\end{equation}
representing the overlap between the vector $g_{t}$ (the vector between our optimal point and our ideal next step) and the error vector $\epsilon(w)_{t}$ as shown in Figure \ref{vectoroverlap}. Given that our dataset is fixed, that our vectors $w_{t}, w^{*} $and $\nabla l(w_{t})$ are fixed, we cannot take an expectation of $cos \theta$ and drop this term. Intuitively for a small move in the weight space, given that our dataset is fixed, we expect our error vector to point in close to the same direction. Bounding the sum as 
\begin{equation}
\sum_{t=1}^{n}|g(w_{t}) ||\epsilon(w)_{t}|\cos \theta_{t} \leq |g(w)_{max} ||\epsilon(w)_{max}|\bigg| \sum_{t=1}^{n}\cos \theta_{t}\bigg|
\end{equation}
which will only concentrate around $0$ if the sum $\frac{1}{n}\sum_{t=1}^{n}cos \theta_{t} \xrightarrow{n \rightarrow \infty} 0$, clearly for a very small move in weight space, where $\cos \theta_{t} \approx \cos \theta_{t+k} \forall k$ this condition is not fulfilled. However it is reasonable to consider that for sufficiently large moves in the weightspace, that the angles between the vectors is uncorrelated, i.e $|\cos \theta_{w_{t}}+\cos \theta_{w_{t+1}}| \propto 2\exp(-|w_{t+1}-w_{t}|/\delta)$, as long as we take sufficiently large step sizes, such that $w_{t+1}-w_{t} \gg \delta$ the bound in our bias term goes to zero, however we do not reduce the second term in our sum optimally. Interestingly, this is exactly the procedure adopted in the recent stochastic weight averaging paper \cite{izmailov2018averaging}, in order to test the hypothesis we...

\subsection{Application to optimization}\label{ssec:application}
Given the stability of the loss surface dynamics in terms of structure and magnitude empirically evidenced in Section \ref{subsec:eigspec_on_cifar10} and the theoretical contributions made in Section \ref{sec:theoreticalcontribution} we learn the optimal parameters for the learning rate and momentum on the Hessian surrogate using the Lanczos Algorithm at that point weight space. We then run SGD or SGDM with the optimal parameters from Equations \ref{eq:alphasgd} \& \ref{eq:alphaandbeta} for the rest of the epoch. The procedure is summarised in Algorithm \ref{alg:ssgd}. When we learn the learning rate only we will denote the the algorithm as SSGD and when we learn the learning rate and the momentum SSGDM, with suffixes for as to whether we use the Gauss-Newton or absolute Hessian approximations.


\begin{algorithm}[tb]
	\caption{SSGD/SSGDM Algorithm}
	\label{alg:ssgd}
	
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} Number of Lanczos steps $m$ and interval $n_l$
		\STATE {\bfseries Output:} SGD learning rate and/or momentum $[\alpha,\beta]$
% 		\STATE Initiate Lanczos algorithm for $m$ steps with $v$
% 		\STATE $\beta = 0, v_{old} = v, \mathbb{V}(:,1) = v$
		\FOR {every $n_l$ training steps}
		\STATE Perform $m$ steps of Lanczos algorithm to learn Ritz-values $\{\lambda_{j}\}_{j=1}^{m}$ of the Gauss-Newton or Absolute Hessian surrogate 
% 		\STATE $\lambda_{max} = \max \{\lambda_{j}\}_{j=1}^{m}$ and compute $\lambda_b$ via Algorithm \ref{alg:learnmeanbulk}
		\IF{ Use SSGD }
	    	\STATE $\alpha = \frac{2}{\lambda_{\mathrm{max}} + \lambda_b}$ with $\lambda_b$ computed by Algorithm \ref{alg:learnmeanbulk}
		    \STATE $\beta = 0 $
		\ELSE
			\STATE $\alpha = \left ( \frac{2}{\sqrt{\lambda_{\mathrm{max}}} + \sqrt{\lambda_b}} \right )^2$
		    \STATE $\beta = \left ( \frac{\sqrt{\lambda_{\mathrm{max}}} - \sqrt{\lambda_b}}{\sqrt{\lambda_{\mathrm{max}}} + \sqrt{\lambda_b}} \right )^2 $
		\ENDIF
% 		\STATE $w = w -\alpha w -\mathbb{V} \mathbb{V}^{T}w$
% 		\STATE $\beta = \sqrt{w^{T}w}$
% 		\STATE $v_{old} = v, v = w/\beta, \mathbb{V}(:,j+1) = v$
% 		\STATE $\mathbb{T}(j,j+1) = \mathbb{T}(j+1,1) = \beta$
		\ENDFOR
% 		%		%\STATE $$
% 		\STATE $[\lambda_{i},e{_{i}}] = eig(\mathbb{T})$ 
% 		\STATE $u_{i} = \mathbb{V} e_{i}, w_{i} = (e_{i}^{T}[1,0,0...0])^{2}$
	\end{algorithmic}
\end{algorithm}

% \begin{algorithm}[tb]
% 	\caption{SSGD/SSGDM Full Algorithm}
% 	\label{alg:ssgd}
	
% 	\begin{algorithmic}[1]
% 		\STATE {\bfseries Input:} Number of Lanczos steps $m$, Gauss-Newton or Absolute Hessian surrogate, Gradient vector $v$
% 		\STATE {\bfseries Output:} Learning Rate and Momentum $]\alpha,\beta]$
% 		\STATE Initiate Lanczos algorithm for $m$ steps with $v$
% 		\STATE $\beta = 0, v_{old} = v, \mathbb{V}(:,1) = v$
% 		\FOR {$j$ in $1,..,m$}
% 		\STATE $w = \mathcal{H}v-\beta v_{old}$
% 		\STATE $\mathbb{T}(j,j) = \alpha = w^{T}v$
% 		\STATE $w = w -\alpha w -\mathbb{V} \mathbb{V}^{T}w$
% 		\STATE $\beta = \sqrt{w^{T}w}$
% 		\STATE $v_{old} = v, v = w/\beta, \mathbb{V}(:,j+1) = v$
% 		\STATE $\mathbb{T}(j,j+1) = \mathbb{T}(j+1,1) = \beta$
% 		\ENDFOR
% 		%		%\STATE $$
% 		\STATE $[\lambda_{i},e{_{i}}] = eig(\mathbb{T})$ 
% 		\STATE $u_{i} = \mathbb{V} e_{i}, w_{i} = (e_{i}^{T}[1,0,0...0])^{2}$
% 	\end{algorithmic}
% \end{algorithm}

\paragraph{Toy example: logistic regression with weight decay on notMNIST}
    We test the validity of our proposed learning and momentum rate scheduler by running SGD and SGDM with logistic regression on the NotMNIST dataset \cite{bulatov2011notmnist}. The logistic regression Hessian is positive semidefinite and we make it positive definite by adding $L2$ weight regularization, $\gamma w^{T}w$. Its Lipcshitz gradient and strong convexity can be calculated analytically, $L \leq \frac{1}{4}\sigma(X^{t}X)+2\gamma$ and $\mu \geq 2\gamma$. Where $\sigma(X^{t}X)$ denotes the maximum eigenvalue of the data matrix $X^{t}X$. We test our learning-rate learner SSGD and learning rate $+$ momentum scheme learner SSGDM by computing the largest eigenvalue and the mean of the bulk every $100$ iterations and then proceeding with either SGD or SGDM, against the equivalent SGD-T and SGDM-T using the theoretically optimal values for general convex functions. We show the results for training and validation error in Figures \ref{fig:toyexample}. Here we see interestingly that the values of $[\mu,L]$ are far too conservative, leading to slow/poor learning for the theoretical case, with the value of momentum given by Equation \ref{eq:alphaandbeta} being so high that the function fails to make significant progress along the gradient direction at all. We note, interestingly, that the training and validation error for SSGDM is even better than SSGD, which suggests improved convergence. 


\begin{figure}[htb!]
	\centering
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=1cm 0cm 0cm 0cm, clip, width=1.0\linewidth]{figures/train_accuracy.eps}
		\caption{Training error} \label{subfig:train_error_toy}
	\end{subfigure}
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=1cm 0cm 0cm 0cm, clip, width=1.0\linewidth]{figures/valid_accuracy.eps}
		\caption{Validation error} \label{subfig:valid_error_toy}
	\end{subfigure}%
	\caption{Training and validation errors achieved on notMNIST by different SGD-based optimiser methods. The subscript \text{T} denotes SGD with learning rate and/or momentum of theoretically derived values.}
	\label{fig:toyexample}
\end{figure}

\paragraph{CNN on CIFAR-10: BasicNet and ResNet}

We apply our proposed approaches to learn the learning rate only (SSGD) and the learning rate and momentum (SSGDM) (Alogrithm \ref{alg:ssgd}) at each epoch to train a basic convolutional neural network (BasicNet), described in Section \ref{subsec:eigspec_on_cifar10} and the ResNet-18 \cite{he2016deep} on the CIFAR-10 dataset using the Tensorflow package. We use $30$ iteration steps for the Lanczos algorithm which runs once at the start of every training epoch. We compared against Adam \cite{kingma2014adam} for which we display the best result obtained after training with learning rate within a grid of $[3 \times 10^{-3} ,3 \times10^{-4},3 \times 10^{-5}]$ \footnote{Logarithmic grid around the default suggested value}, and stochastic gradient descent with momentum (SGDM) as well as pure stochastic gradient descent (SGD) for which we display the best results obtained after training with learning rate in the range $[0.1, 0.01, 0.001, 0.0001]$. For all the optimizers, we adopt a batch size of $128$ and use the cross entropy loss as the training objective. 

We show our results on both training and validation loss on the BasicNet in Figure \ref{fig:basicnet_cifar10_opt}. We see all variants of our algorithm outperform the best SGD and Adam in terms of the training loss while performing as well as them in the validation loss. For the ResNet, with results shown in Figure \ref{fig:ResNet_cifar10_opt}, here we compare the variants of our algorithms against the state of the art expert SGD tuning schedule, which has a momentum of $0.9$ and $3$ epochs of warm start with a learning rate of $0.001$, $80$ epochs of $0.1$, $10$ epochs of $0.01$, $27$ epochs of $0.001$ and a final learning rate of $0.0001$ for the rest of the training, with the same schedule without momentum also plotted. Here we can see that the absolute Hessian approximation with learned momentum performs best out of our methods, incredibly close to the expert scheduled SGD and even converges faster in the validation loss.

\begin{figure}[htb!]
	\centering
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.0cm 0cm 0.0cm 0.5cm, clip, width=1.0\linewidth]{figures/CIFAR10_BasicNet_BN_train.eps}
		\caption{Training loss}
	\end{subfigure}
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.0cm 0cm 0.0cm 0.5cm, clip, width=1.0\linewidth]{figures/CIFAR10_BasicNet_BN_valid.eps}
		\caption{Validation loss}	
	\end{subfigure}%
	\caption{Training and validation losses for the BasicNet.}
	\label{fig:basicnet_cifar10_opt}
\end{figure}

\begin{figure}[htb!]
	\centering
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.0cm 0cm 0.0cm 0.5cm, clip, width=1.0\linewidth]{figures/CIFAR10_ResNet_BN_train.eps}
		\caption{Training loss}
	\end{subfigure}
	\begin{subfigure}{0.45\linewidth}
		\centering
		\includegraphics[trim=0.0cm 0cm 0.0cm 0.5cm, clip, width=1.0\linewidth]{figures/CIFAR10_ResNet_BN_valid.eps}
		\caption{Validation loss}	
	\end{subfigure}%
	\caption{Training and validation losses for the ResNet-18.}
	\label{fig:ResNet_cifar10_opt}
\end{figure}




% \begin{figure}[H]
% 	\centering
% 	\begin{subfigure}{0.45\linewidth}
% 		\centering
% 		\includegraphics[trim=1cm 8.5cm 2cm 8.43cm, clip, width=1.0\linewidth]{figures/resnet0itbn.pdf}
% 		\caption{ResNet BN: Iteration 0}
% 	\end{subfigure}
% 	\hspace{5pt}
% 	\begin{subfigure}{0.45\linewidth}
% 		\centering
% 		\includegraphics[trim=1cm 8.5cm 2cm 8.43cm, clip, width=1.0\linewidth]{figures/resnet468itbn.pdf}
% 		\caption{ResNet BN: Iteration 468}	
% 	\end{subfigure}%
% 	\vspace{5pt}
	
% 	\begin{subfigure}{0.45\linewidth}
% 		\centering
% 		% 		 trim={<left> <lower> <right> <upper>}
% 		\includegraphics[trim=1cm 8.5cm 2cm 8.43cm, clip, width=1.0\linewidth]{figures/resnet936itbn.pdf}
% 		\caption{ResNet BN: Iteration 936}	
% 	\end{subfigure}%
% 	\hspace{5pt}
% 	\begin{subfigure}{0.45\linewidth}
% 		\centering
% 		\includegraphics[trim=1cm 8.5cm 2cm 8.43cm, clip, width=1.0\linewidth]{icml2018_style/figures/resnet1872itbn.pdf}
% 		\caption{ResNet BN: Iteration 1872}	
% 	\end{subfigure}%
% 	\vspace{5pt}
% 	\vspace{5pt}
	
% 	\caption{Eigen-spectra of Gauss Newton Matrices for a Resnet-18 Network on Cifar-10, trained using SGD with learning rate of $0.001$. }\label{fig:cifarresnet18}
% \end{figure}







% \begin{figure}[htb!]
% 	\centering

% 	\caption{The effect of using low momentum and high momentum on training and validation loss of the ResNet-18.}
% 	\label{fig:resnet_lowvshigh}
% \end{figure}

==> math.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vphi{{\bm{\phi}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\vtheta{{\bm{\theta}}}
\def\vdelta{{\bm{\delta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> method.tex <==

\section{Neural network loss Hessian}\label{sec:spectralimplication}
However, in reality the neural network loss surface is neither convex, nor directly accessible. Indeed, even if it were to be accessible, the errors introduced by finite batch size, shown in section \ref{subsec:spectralimplications} would still need to be compensated for. Our work offers a principled framework which addresses all these drawbacks in a unified manner.
In order to work within the convex framework set out in Section \ref{sec:quadraticformulae}, we will use positive definite approximation of the Hessian which we will denote as $\bar{H}$.  We consider two positive definite approximations to the Hessian commonly used in Deep Learning optimization, the Generalised Gauss Newton (GGN)\cite{schraudolph2002fast, martens2010deep} and the Absolute Hessian, which consists of leaving the Hessian eigenvectors unchanged  and taking the absolute value of the eigenvalues\cite{dauphin2014identifying}, i.e $\bar{H} = \sum_{i=1}^{n}|\lambda_{i}||\phi_{i}\rangle\langle\phi_{i}|$, where $[\lambda_{i}, |\phi_{i}\rangle]$ are the eigenvalues and eigenvectors respectively of the Hessian $H \in \mathbb{R}^{n\times n}$ of the loss $L$. In general, both methods can be viewed as trust-regions methods for the losses commonly used in the DNN litterature (\emph{e.g} softmax or $L_2$)\cite{pascanu2013revisiting, pascanu2014saddle}. Both approximations are saddle point avoidant and the GGN is the only convex quadratic approximation which does not change the objective functions minimia \cite{chen2011Hessian}. Subscripts $_{G}$ or $_{H}$ would refer to either Gauss-Newton or Absolute Hessian variants in the rest of the paper. Our theoretical arguments are invariant to the use of a positive definite surrogate and so for simplicity we will in general stick to the use of GGN unless otherwise specified. 

\subsection{Spectral implications of finite batch-size}
\label{subsec:spectralimplications}
A naive application of Eq.\ref{eq:alphaandbeta} and Eq.\ref{eq:alphasgd} would have us estimate the largest and smallest non zero eigenvalues of the spectrum. However in the typical Deep Learning scenario where we work with a batch size far smaller than our total parameter number $T \ll N$, it is expected that our observed "empirical" GGN matrix generated using $T$ samples deviates significantly from it's "true" counterpart obtained from the whole dataset. 

Firstly, the rank of a matrix the GGN matrix scales is equal to the   the batch size $T$ multiplied by the number of classes. This can be seen from its definition \cite{schraudolph2002fast}
\begin{equation}
    \text{rank}(G) = \text{rank}\bigg(\frac{1}{T}\sum_{i}^{T}J^{T}_{f,i}H_{l,i}J_{f,i}\bigg) \leq T\times n_{c}
\end{equation}
Where $J_{f,i}$ is the Jacobian of the output with respect to the parameters for the $i$'th data-point, and similarly $H_{L,i}$ is the hessian of $L(y,z)$ with respect to the output $z$. $n_{c}$ is the number of classes. Clearly the rank of a product is the minimum rank of its products so upper bounded by the $\text{rank}(H_{L}) = n_{c}$ and the rank of $T$ such matrices is again upper bounded by $T$ times the original upper bound.

{\color{red} We need to bring back the old argument}. Hence the empirical Gauss-Newton will always have a minimum eigenvalue of $\lambda_{n} = 0$, independently of whether its "true" counterpart does. We call these eigenvalues "ghosts" because much like their fantastical counterpart, many of them are largely due to measurement error. 

To show that even accounting for this $0$ spike is not enough, as other small eigenvalues will also be underestimated in magnitude, we consider the $L_2$ loss between the true GGN matrix $G$, and our estimator thereof $\Xi(M)$
\begin{equation}
\argmin_{\Xi(M)}||G-\Xi(M)||_2
\end{equation}
by making the assumption that the estimator is rotationally invariant \cite{bun2016rotational}, which means that the estimator shares the same eigenbasis as the empirical Gauss-Newton, gives the optimal estimator of the eigenvalues $ \Hat{\xi}_{i}$ as
\begin{equation}
\hat{\xi}_{i} = \sum_{j=1}^{N}\langle u_{i}|\hat{u}_{j}\rangle^{2}\lambda_{j}
\end{equation}
Where $u_{i}$ denotes the un-perturbed eigenvectors of the true Gauss-Newton and $(\hat{u}_{j}$, $\lambda_{j}) \in \mathbb{R}^{N}\times\mathbb{R}$ denotes the perturbed (eigenvectors,eigenvalues) of the empirical Gauss-Newton. This shows that small observed eigenvalues should be increased, since there is a non zero contribution from the larger eigenvalues as the overlap is $\geq 0$, and large eigenvalues should be decreased.

%Furthermore, as shown in (CITE WHY HESSIA ARE NOT THAT SINGULAR FUTURE PAPER) for convex quadratics such as the generalised gauss newton (GGN) for $N>T$ we expect $N-T$ ghost eigenvalues and by noting that the Hessian can be seen as a small perturbation of the GGN we expect the empirical Hessian for $N\gg T$ to be highly degenerate even when the true Hessian is not.
The two aforementioned problems put us into a seeming double bind. The smallest non zero eigenvalue of the true Gauss-Newton in its empirical counterpart is attracted to $0$ by spectral broadening and may likely converge to $0$, as shown in Figure \ref{fig:marcenkopastur}. This would make it hard to distinguish from the "ghost" eigenvalues. Further even if the empirical Gauss-Newton has a seperation between $\lambda_{n-k}>0$ and $0$, the convergence of iterative methods depend on the eigengaps \cite{meurant2006lanczos} and hence it will struggle to distinguish between different values within the bulk, especially for a small number of Lanczos steps. This makes direct estimation of $\lambda_{n-k}$ impossible. We provide a method to avoid this problem in the next sub-section.

\subsection{Model for learning the smallest non zero eigenvalue}
\label{sec:theoreticalcontribution}
In the case where the Gauss-Newton can be assumed to be a scalar multiple of the identity matrix, the exact analytical form of the broadened spectrum is known. The resulting limiting spectral density, (i.e. $T,N \rightarrow \infty, N/T = q$) is known and is given by the Marcenko-Pastur equation \cite{bun2017cleaning}
\begin{equation}
\label{eq:marcenkopastur}
\begin{aligned}
& \mu(A) = (1-\frac{1}{q})\mathbbm{1}_{0\in A}+\nu(A), \thinspace  \text{if} \thinspace q>1\\
& d\nu(x) = \frac{1}{2\pi\sigma^{2}}\frac{\sqrt{(\lambda_{+}-x)(x-\lambda_{-})}}{\lambda x}\mathbbm{1}_{[\lambda_{-},\lambda_{+}]}dx.
\end{aligned}
\end{equation}

\begin{figure}
    \centering
		\includegraphics[trim=1cm 0.2cm 0cm 0cm, clip, width=1\linewidth]{figures/MP_demo_plots.eps}
		\caption{Effect of spectral broadening on a simple spectrum}
    \label{fig:marcenkopastur}
\end{figure}
For finite rank perturbations of the identity, the eigenvalues sufficiently far from the bulk are minimally perturbed and the rest follow the Marcenko-Pastur equation \cite{bun2017cleaning,baik2004eigenvalues,baik2006eigenvalues}. We visualize this effect in Figure \ref{fig:marcenkopastur}, where the bulk of the spectral mass is at $\lambda=1$ and there are a few small perturbations, as we move from the large sample regime $T \gg N$, to the large dimension limit \cite{baik2006eigenvalues} $T = \mathcal{O}(N)$ the spectral mass at $\lambda=1$ spreads out into the Marcenko-Pastur distribution shown in Equation \eqref{eq:marcenkopastur} and the well seperated outlier eigenvalues are minimally perturbed (not shown). In the limit $T \ll N$ we would have a massive spectral spike at $\lambda=0$ as mentioned earlier in this section (also not shown). The mean of the Marcenko-Pastur equation \eqref{eq:marcenkopastur} is given by $\sigma^{2}$, which, for the special case of the identity matrix, is $1$ and hence by discounting the excess zero mode (caused by using a small sample $T < N$) and eigenvalues well seperated from the bulk, the mean of the remaining continous spectrum constitutes our Marcenko-Pastur estimation of the lowest eigenvalue $\lambda_{b} \approx \lambda_{n}$. We demonstrate an example of what we would expect from a broadened spectrum with a few well separated outlier eigenvalues in Figure \ref{fig:marcenkopastur}, along with the cleaned spectrum from our procedure. We detail the procedure in Algorithm \ref{alg:learnmeanbulk}. Crucial to the procedure is the removal of the spectral mass corresponding to the "ghost" eigenvalues, which we do by removing the Ritz value of smallest absolute magnitude and estimating the number of eigenvalues well seperated from the bulk, for which we derive a procedure in the next section.
%We further note than in the less restrictive approximation of simply assuming bounded $4$'th moments of the input distribution (IS THE MARCENKO-PASTUR ALSO RECOVERED OR JUST THE CONTINOUS SPECTRUM CHECK UNIVERSALITY)
\subsection{Heuristic for the number of and values of outliers}
\label{ssec:outliernumber}
%Now that we can estimate the smallest eigenvalue of the spectrum, we turn to the opposite task of finding its highest value. 
If we consider a block-diagonal approximation to the Gauss-Newton \cite{botev2017practical}, which constitutes the Gauss-Newton approximation to a layer-wise independent loss function. As all the Gauss-Newton eigenvalues are positive, the average element in each layer $\mu_{l}$ must also be positive. This can be seen by taking the vector of ones $\langle 1 |$ and calculating $\langle 1 | G | 1 \rangle$. As the eigenvalues of a block diagonal matrix are simply the union of eigenvalues of the blocks, the same argument holds true for the individual blocks. Separating the positive mean value for each layer $l$, $\mu_{l}$ from the rest of the matrix gives us
\begin{equation}
   \begin{aligned}
G = & \begin{bmatrix} \mu_{1} \begin{bmatrix}
1 & 1  \\
1 & \ddots \\
\end{bmatrix} & 0 \\
0 & \mu_{2} \begin{bmatrix}
1 & 1  \\
1 & \ddots \\
\end{bmatrix} & 
\end{bmatrix} + \tilde{G}
\end{aligned} 
\end{equation}
Where $\tilde{G}$ is now a block-diagonal matrix of mean $0$ in the blocks. The matrix of all ones contributes a singular eigenvalue of magnitude $n_{l} \times \mu_{l}$ to the eigen-spectrum, where $n_{l}$ is the number of elements in the layer $l$ . 
\begin{equation}
    G|1\rangle_{n_{l}} = n_{l}\mu_{l} + \tilde{G}|1\rangle_{n_{l}} = n_{l}\mu_{l} + \sum_{l}\tilde{G}_{il}
\end{equation}
Hence assuming the elements of the blocks to be independent bounded variables \footnote{For large over paramterised networks we can assume the Hessian elements to have some degree of independence}, up to order $\sqrt{1/n_{l}}$ there are $j$ eigenvalues of size $n_{l}\mu_{l}$, $\forall l\leq j$, where $j$ is the number of layers. Under the same assumptions, the next largest eigenvalue within the blocks scales as $\mathcal{O}(2\sigma_{l}\sqrt{n_{l}})$ \cite{furedi1981eigenvalues}. Hence, so long as $\text{argmax}_{i} (2\sigma_{i}\sqrt{n_{i}} )\ll \text{argmin}_{i} (n_{i}\mu_{i})$ there are $j$ well separated eigenvalues, where $\sigma_{i}$ denotes the standard deviation of the elements in the submatrix $i$. This gives us an approximation of $j$ outlier eigenvalues for the Gauss-Newton.



\begin{algorithm}[htb!]
	\caption{Mean of the bulk learned with a random vector}
	\label{alg:learnmeanbulk}
	\begin{algorithmic}
		\STATE {\bfseries Input:} Lanczos Ritz-values/vectors $\lambda_{i},{\mu}_{i}, \forall i \leq m$, number of Layers $l$
		\STATE $w_{i} = {\mu}_{i}[1]^{2}$
		\STATE $w_{j} = \text{argmax}_{i}w_{i}$
		\STATE $\tilde{w} = \frac{w[l+1:j-1]}{\sum_{j=0}w[n_{l}:j-1]}$
		\STATE {\bfseries Output:} $\lambda_{b} = \sum_{i=n_{l}+1}^{m-l-j-2}\lambda_{i}\tilde{w}_{i}$
	\end{algorithmic}
\end{algorithm}
%(CONSIDER GERSHGORIN BOUND ON THE MOD OF A RANDOM VARIABLE WITH SIGMA). 
%In order to experimentally validate the above intuition we train a $9$ layer basic convolutional neural network with SGD using generic parameters of $alpha = 0.01, \beta = 0.9$ with a batch-size of $T=128$ and plot the approximate empirical spectral density of the Gauss-Newton with $0$ mode removed at regular intervals using the Lanczos-algorithm, in figure \ref{fig:cnnexp}. We note exceptional agreement with our naive independent layer and independent element assumption model with even the number of ourliers at the $0$'th iteration being $\mathcal{O}(10)$ and there being exactly $9$ outliers in the later iterations for the non-batch norm network. We note that when using batch-norm the number of outliers increases and their seperation from the bulk is less pronounced. This is to be expected because the inputs are normalised, we leave a more thorough treatment as future work.


==> related_work.tex <==
\section{Related work} The largest Hessian eigenvalue has been used to learn the learning rate \cite{lecun1993automatic}, using the power iteration method which has a significantly worse convergence as compared to Lanczos method \cite{meurant2006lanczos}. Methods to adapt the the learning rate per layer or globally using diagonal approximations to the Hessian have been suggested \cite{schaul2013nopesky}. We note that neural network Hessian are often strongly non-diagonal \cite{Martens2016}. Furthermore, none of these works look at learning the global momentum term, which allows for more aggressive learning rates and improved performance. Full second order methods \cite{martens2010deep} reduce the need for learning rate schedules and function without including momentum, however the extra computational cost is several orders of magnitude higher per iteration and we do not find the performance justifies the cost compared with fine tuned momentum \cite{sutskever2013importance}, for which we propose a method. 
